Universal Lossless Compression of Graphical Data

Graphical data is comprised of a graph with marks on its edges and vertices. The mark indicates the value of some attribute associated to the respective edge or vertex. Examples of such data arise in social networks, molecular and systems biology, and web graphs, as well as in several other application areas. Our goal is to design schemes that can efficiently compress such graphical data without making assumptions about its stochastic properties. Namely, we wish to develop a universal compression algorithm for graphical data sources. To formalize this goal, we employ the framework of local weak convergence, also called the objective method, which provides a technique to think of a marked graph as a kind of stationary stochastic processes, stationary with respect to movement between vertices of the graph. In recent work, we have generalized a notion of entropy for unmarked graphs in this framework, due to Bordenave and Caputo, to the case of marked graphs. We use this notion to evaluate the efficiency of a compression scheme. The lossless compression scheme we propose in this paper is then proved to be universally optimal in a precise technical sense. It is also capable of performing local data queries in the compressed form.

==> Alternate_proof_with_common_m_sub_n.tex <==
\section{Alternate proof with common $m_n$}
%\label{sec:proof-theorem-gen-BC-properties}

We prove the invariance under the change of the sequence $\bu_n$. 

\begin{prop}
  \label{prop:bch-invariant-un}
Assume $\mu \in \mP(\mGb_*)$ is given such that $0<\deg_x(\mu) <\infty$ for all $x \in \Xi$ and $\vtype_t(\mu) > 0$ for all $t \in \vermark$.  Additionally, assume the degree vector $\bd=(d_x)_{x \in \edgemark}$ together with the probability distribution $\pi=(\pi_t)_{t \in \vermark}$ are given such that $0<d_x<\infty$ for all $x \in \edgemark$ and $\pi_t > 0$ for all $t \in \vermark$. 
Fix sequences $\bm_n, \bu_n,\tilde{\bu}_n$ such that $ \bm_n(x)/n \rightarrow d_x/2$ for all $x \in \edgemark$ and for all $t \in \vermark$, $\lim_{n \rightarrow \infty} \bu_n(t) / n = \lim_{n \rightarrow \infty} \tilde{\bu}_n(t) / n = \pi_t$. Let $\bchover^{(1)}_{\bd, \pi}(\mu)$ be the entropy in definition~\ref{def:bch-color} resulting from the sequence $\bu_n$ and $\bchover^{(2)}_{\bd, \pi}(\mu)$ is the same object resulting from the sequence $\tilde{\bu}_n$ (where in both scenarios we use $\bm_n$ for edge counts). Then, we have $\bchover^{(1)}_{\bd, \pi}(\mu) = \bchover^{(2)}_{\bd, \pi}(\mu)$. Moreover, if $\bchunder^{(1)}_{\bd, \pi}(\mu)$ and $\bchunder^{(2)}_{\bd, \pi}(\mu)$ are defined similarly, we also have $\bchunder^{(1)}_{\bd, \pi}(\mu) = \bchunder^{(2)}_{\bd, \pi}(\mu)$. 
\end{prop}

\marginpar{\color{red} Note that Definition ~\ref{def:bch-color}  discusses
$\bchover^{(1)}_{\bd, \pi}(\mu, \epsilon)$ and one needs to let $\epsilon \to 0$.}

\begin{rem}
  Although we have not assumed in the above statement that $d_x = \deg_x(\mu)$ for all $x \in \edgemark$, Proposition~\ref{prop:deg-not-match-bch-inf} in Appendix~\ref{sec:cond-BC-infty} implies that  if $d_x \neq \deg_x(\mu)$ for some $x \in \edgemark$, $\bchover^{(1)}_{\bd, \pi}(\mu) = \bchover^{(2)}_{\bd, \pi}(\mu) = \bchunder^{(1)}_{\bd, \pi}(\mu) = \bchunder^{(2)}_{\bd, \pi}(\mu) = -\infty$.
\end{rem}

\begin{proof}
Recall from \eqref{eq:vertype-probability} that $\vtype_t(\mu)$ is the probability under $\mu$ that the mark of the root is $t$. 
We claim that if $\pi_{\hat{t}} \neq \vtype_{\hat{t}}(\mu)$ for some $\hat{t} \in \vermark$, then $\bchover^{(1)}_{\bd, \pi}(\mu) = \bchover^{(2)}_{\bd, \pi}(\mu) = \bchunder^{(1)}_{\bd, \pi}(\mu) = \bchunder^{(2)}_{\bd, \pi}(\mu) = -\infty$. For instance, assume $\bchover^{(1)}_{\bd, \pi}(\mu) > -\infty$. A diagonalization argument implies that there exists an $M > -\infty$ together with sequences $n_k$ and $\epsilon_k$ such that as $k \rightarrow \infty$, $n_k \rightarrow \infty$ and $\epsilon_k \rightarrow 0$, and for all $k$.
\begin{equation*}
    \frac{\log |\mG^{(n_k)}_{\bm_{n_k}, \bu_{n_k}}(\mu, \epsilon_k)| - \norm{\bm_{n_k}}_1 \log n}{n_k} > M.
\end{equation*}
This in particular implies that the set $\mG^{(n_k)}_{\bm_{n_k}, \bu_{n_k}}(\mu, \epsilon_k)$ is not empty for every $k$. If $\bG_k$ is an arbitrary member of $\mG^{(n_k)}_{\bm_{n_k}, \bu_{n_k}}(\mu, \epsilon_k)$, since $\epsilon_k\rightarrow 0$, $\dlp(U(\bG_k), \mu) \rightarrow 0$. As the \LP metric metrizes the topology of weak convergence in $\mGb_*$, this means that $U(\bG_k)$ converges weakly to $\mu$. 
Now, define the function $f$ on $\mGb_*$ to be the indicator function of the mark of the root being $\hat{t}$, i.e. $f([\bG, o]) := \oneu{\tau_{\bG}(o) = \hat{t}}$. Since $f$ is bounded and continuous on $\mGb_*$ and $U(\bG_k) \Rightarrow \mu$, it must be the case that $\int f d U(\bG_k) \rightarrow \int f d \mu$. But $\int f dU(\bG_k) = \bu_{n_k}(\hat{t})/n_k$ while $\int f d \mu = \vtype_{\hat{t}}(\mu)$. This is a contradiction since $\bu_{n_k}(\hat{t})/n_k \rightarrow \pi_{\hat{t}} \neq \vtype_{\hat{t}}(\mu)$. Therefore, $\bchunder^{(1)}_{\bd, \pi}(\mu) \leq \bchover^{(1)}_{\bd, \pi}(\mu) = -\infty$. Similarly, $\bchunder^{(2)}_{\bd, \pi}(\mu) \leq \bchover^{(2)}_{\bd, \pi}(\mu) = -\infty$. Thus far, we have shown that if $\pi_{\hat{t}} \neq \vtype_{\hat{t}}(\mu)$ for some $\hat{t} \in \vermark$,  $\bchover^{(1)}_{\bd, \pi}(\mu) = \bchover^{(2)}_{\bd, \pi}(\mu) = \bchunder^{(1)}_{\bd, \pi}(\mu) = \bchunder^{(2)}_{\bd, \pi}(\mu) = -\infty$, and the statement of the above proposition holds.\footnote{It is fruitful to emphasize that a similar argument does not work for edge counts, i.e. to show that if $d_{x^*} \neq \deg_{x^*}(\mu)$ for some $x^* \in \edgemark$, $\bchover_{\bd, \pi}(\mu) = -\infty$. The reason is that although the function $f$ on $\mGb_*$ defined as $f([\bG, o]) = \deg_{\bG}(o;x^*)$ is continuous, it is not bounded. Thereby, one can not argue that the integral of $f$ against $U(\bG_k)$, which is $2 \bm_n(x^*) / n$, converges to $\int f d \mu = \deg_{x^*}(\mu)$. In fact, even if we truncate $f$ to make it bounded, by sending the truncation level to infinity and using monotone convergence theorem, we get $\liminf \bm_n(x^*)/n \geq \deg_{x^*}(\mu)$. See Proposition~\ref{prop:deg-not-match-bch-inf} in Appendix~\ref{sec:cond-BC-infty}.} Hence, it remains to prove the statement under the assumption that $\pi_t = \vtype_t(\mu)$, for all $t \in \vermark$. 

Write $\vermark$ as $ \{t_1, \dots, t_{|\vermark|} \}$. Define
\begin{equation*}
  I^{(n)}_{t_1} := \{1, \dots, \bu_n(t_1) \},
\end{equation*}
and
\begin{equation*}
  I^{(n)}_{t_l} := \left \{ 1 + \sum_{i=1}^{l-1} \bu_n(t_i), \dots, \sum_{i=1}^l \bu_n(t_i)\right  \} \qquad 2 \leq l \leq |\vermark|.
\end{equation*}
Similarly, let
\begin{equation*}
  \tilde{I}^{(n)}_{t_1} := \{1, \dots, \tilde{\bu}_n(t_1) \},
\end{equation*}
and
\begin{equation*}
  \tilde{I}^{(n)}_{t_l} := \left \{ 1 + \sum_{i=1}^{l-1} \tilde{\bu}_n(t_i), \dots, \sum_{i=1}^l \tilde{\bu}_n(t_i)\right  \} \qquad 2 \leq l \leq |\vermark|.
\end{equation*}
Now, for an arbitrary graph $\bG \in \mG^{(n)}_{\bm_n, \bu_n}(\mu, \epsilon)$, 
one can find a permutation $\pi \in S_n$ such that in $\pi \bG$, all vertices in $I^{(n)}_{t_i}$ have mark $t_i$, for $1 \leq i \leq |\vermark|$. Then, $U(\pi \bG) = U(\bG)$. Let $\mG'^{(n)}_{\bm_n, \bu_n}$ be the subset of $\mG^{(n)}_{\bm_n, \bu_n}$ containing graphs in which all  vertices in $I^{(n)}_{t_i}$ have mark $t_i$,  $1 \leq i \leq |\vermark|$. Moreover, let $\mG'^{(n)}_{\bm_n, \bu_n}(\mu, \epsilon)$ be the set of graphs $\bG$ in $\mG'^{(n)}_{\bm_n, \bu_n}$ such that $\dlp(U(\bG), \mu) < \epsilon$. Let $\mG'^{(n)}_{\bm_n, \tilde{\bu}_n}$ and $\mG'^{(n)}_{\bm_n, \tilde{\bu}_n}(\mu, \epsilon)$ be defined similarly with $\bu_n$ being  replaced by  $\tilde{\bu}_n$. 

Let $S_{\bu_n}$ denote the subgroup of $S_n$ consisting of permutations $\pi$ such that $\pi I^{(n)}_{t_i} = I^{(n)}_{t_i}$, for $1 \leq i \leq |\vermark|$. Additionally, fix $M = \frac{n!}{\prod_{i=1}^{|\vermark|} \bu_n(t_i)!}$ permutations $\pi_1, \dots, \pi_M$ in $S_n$ such that $S_n$ is the disjoint union of $\pi_k S_{\bu_n}$ for $1 \leq k \leq M$. The above discussion then implies that $\mG^{(n)}_{\bm_n, \bu_n}(\mu, \epsilon)$ is the disjoint union of $\pi_k \mG'^{(n)}_{\bm_n, \bu_n}(\mu, \epsilon)$ for $1 \leq k \leq M$, where $\pi_k \mG'^{(n)}_{\bm_n, \bu_n}(\mu, \epsilon)$ denotes the action of $\pi_k$ on all graphs in $\mG'^{(n)}_{\bm_n, \bu_n}(\mu, \epsilon)$ (recall the notion of the action of a permutation on a graph from Section~\ref{sec:preliminaries}). This together with the fact that $\bu_n(t) / n \rightarrow \pi_t$ for all $t \in \vermark$ implies 
\begin{equation*}
  \log | \mG^{(n)}_{\bm_n, \bu_n}(\mu, \epsilon)| = \log |\mG'^{(n)}_{\bm_n, \bu_n}(\mu, \epsilon)| + nH(\pi) + o(n),
\end{equation*}
and similarly,
\begin{equation*}
  \log | \mG^{(n)}_{\bm_n, \tilde{\bu}_n}(\mu, \epsilon)| = \log |\mG'^{(n)}_{\bm_n, \tilde{\bu}_n}(\mu, \epsilon)| + nH(\pi) + o(n).
\end{equation*}
This shows that if we define 
\begin{equation*}
  \bchover'^{(1)}_{\bd, \pi}(\mu) := \lim_{\epsilon\downarrow 0} \limsup_{n\rightarrow \infty} \frac{\log |\mG'^{(n)}_{\bm_n, \bu_n}(\mu, \epsilon) | - \norm{\bm_n}_1\log n}{n},
\end{equation*}
and 
\begin{equation*}
  \bchover'^{(2)}_{\bd, \pi}(\mu) := \lim_{\epsilon\downarrow 0} \limsup_{n\rightarrow \infty} \frac{\log |\mG'^{(n)}_{\bm_n, \tilde{\bu}_n}(\mu, \epsilon) | - \norm{\bm_n}_1\log n}{n},
\end{equation*}
and  similarly $\bchunder'^{(1)}_{\bd, \pi}(\mu)$ and $\bchunder'^{(2)}_{\bd, \pi}(\mu)$, it suffices to show that $  \bchover'^{(1)}_{\bd, \pi}(\mu) =   \bchover'^{(2)}_{\bd, \pi}(\mu)$ and $\bchunder'^{(1)}_{\bd, \pi}(\mu) = \bchunder'^{(2)}_{\bd, \pi}(\mu)$. In order to do so, we define a mapping $F_n: \mG'^{(n)}_{\bm_n, \bu_n} \rightarrow \mG'^{(n)}_{\bm_n, \tilde{\bu}_n}$ in the following way:
given a graph $\bG \in \mG'^{(n)}_{\bm_n, \bu_n}$, for all vertices $1 \leq i \leq n$ in $\bG$, there is a unique $1 \leq j_i \leq |\vermark|$ such that $i \in \tilde{I}^{(n)}_{t_{j_i}}$. The mapping $F_n$ then changes the mark of all vertices $1 \leq i \leq n$ to $t_{j_i}$, and leaves edges and their marks untouched. 
See Figure~\ref{fig:Fn-vertex-mark-change} for an illustration.
Note that $F_n$ is a bijective mapping. 
 Our goal is to show that when $\epsilon$ is small enough and $n$ is large enough, for a sufficiently large fraction of graphs $\bG \in \mG'^{(n)}_{\bm_n, \bu_n}(\mu, \epsilon)$, $F_n(\bG)$ is contained in $\mG'^{(n)}_{\bm_n, \tilde{\bu}_n}(\mu, \epsilon')$, for $\epsilon'$ slightly larger than $\epsilon$. 

\begin{figure}
  \centering
  \begin{tikzpicture}
    \begin{scope}[xshift=-3cm,scale=0.7]
      \node[Node,label={above:1}] (n1) at (-1,1) {};
      \node[Node,label={above:2}] (n2) at (1,1) {};
      \node[Node2,label={below:3}] (n3) at (-1,-1) {};
      \node[Node2,label={below:4}] (n4) at (1,-1) {};
      \draw[Cyan,thick] (n2) -- (n1) -- (n4) -- (n3);
      \draw[Orange,densely dotted, very thick] (n2) -- (n3);
    \end{scope}
    \node at (0,0.5) {$F_n$};
    \draw[->] (-0.5,0) -- (0.5,0);
    \begin{scope}[xshift=3cm,scale=0.7]
      \node[Node,label={above:1}] (n1) at (-1,1) {};
      \node[Node2,label={above:2}] (n2) at (1,1) {};
      \node[Node2,label={below:3}] (n3) at (-1,-1) {};
      \node[Node2,label={below:4}] (n4) at (1,-1) {};
      \draw[Cyan,thick] (n2) -- (n1) -- (n4) -- (n3);
      \draw[Orange,densely dotted, very thick] (n2) -- (n3);
    \end{scope}
  \end{tikzpicture}
  \caption{\label{fig:Fn-vertex-mark-change} An illustration of the action of the function $F_n$. In this example, $n=4$,
$\edgemark = \{\text{\color{Cyan} Cyan (solid)}, \text{\color{Orange} Orange (dotted)} \}$,
$\vermark = \{t_1 = \bullet, t_2 = \blacksquare\}$, $\bu_n(t_1) = \bu_n(t_2) = 2$, $\tilde{\bu}_n(t_1) = 1, \tilde{\bu}_n(t_2) = 3$, $\bm_n({\color{Cyan} \text{Cyan}}) = 3$ and $\bm_n({\color{Orange} \text{Orange}}) = 1$. Note that the mark of vertex $2$ has changed from $\bullet$ to $\blacksquare$.}
\end{figure}

Let $\epsilon_0 = \frac{1}{6} \wedge \frac{1}{2} \min_{t \in \vermark} \pi_t$. Note that $\epsilon_0 > 0$ since by assumption $\pi_t > 0$ for all $t$. Choose $0 < \epsilon < \epsilon_0$ and fix an integer $k$ such that $\epsilon < 1/(1+k) < 1/k < 2 \epsilon$ (which is possible when $\epsilon< 1/6$). For $t \in \vermark$ and positive integer $r$, let $A^{t}_{k, r}$ be the set of $[\bG, o] \in \mGb_*$ such that the mark of the root is $t$ and there are at most $r$ many vertices up to depth $k$. Since the elements of $\mGb_*$ are locally finite, the probability of the mark of the root being $t$ is $\pi_t$, and $\epsilon<\min_{t \in \vermark} \pi_t$, we can choose $r_t$ such that $\mu(A^t_{k, r_t}) \geq \pi_t - \epsilon$. 
For a marked graph $\bG \in \mG'^{(n)}_{\bm_n, \bu_n}$ and $t \in \vermark$, let
\begin{equation*}
  J^{(n)}_t(\bG) := \{ i\in I^{(n)}_t: [\bG, i]_k \in A^t_{k, r_t} \}.
\end{equation*}

For $t \in \vermark$, let $Y^{(n)}_t = I^{(n)}_t \setminus \tilde{I}^{(n)}_t$, which is effectively the set of vertices with mark $t$ such that their mark is changed after applying $F_n$. Indeed, $Y^{(n)}_t$ only dependent on $\bu_n$ and $\tilde{\bu}_n$.
% (for instance, if $\vermark = \{a, b, c\}$, $n=5$, $\bu_n(a)= 1$, $\bu_n(b) = \bu_n(c) = 2$, $\tilde{\bu}_n(a)= \tilde{\bu}_n(b) = 2$ and $\tilde{\bu}_n(c) = 1$, then $Y^{(n)}_a = \emptyset$, $Y^{(n)}_b = \{2\}$ and $Y^{(n)}_c = \{4\}$). 
let $Y^{(n)} = \cup_{t \in \vermark} Y^{(n)}_t$. 
Moreover, due to the assumption that for all $t$, both $\bu_n(t)/ n$ and $\tilde{\bu}_n(t)/n$ converge to the same $\pi_t$, $|Y^{(n)}|=\sum_{t \in \vermark} |Y^{(n)}_t| = o(n)$. 
%which is essentially the set of vertices with mark $t$ in $\bG$ which do not have more than $r_t$ many nodes in their $k$--neighborhood. Note that if a vertex with mark $t$ which is going to change its mark (i.e. is in the set $Y^{(n)}_t$) is also in the set $J^{(n)}_t(\bG)$, since its local neighborhood up to depth $k$ does not contain more than a fixed number ($r_t$) many vertices, where $r_t$ does not depend on $n$, changing its color should not change $U(\bG)$ very much. To make this precise, 
We call $\bG \in \mG'^{(n)}_{\bm_n, \bu_n}$ to be \emph{good} if $Y^{(n)}_t \subseteq J^{(n)}_t(\bG)$ for all $ t\in \vermark$. Let $\bG' = F_n(\bG)$. Since the mark of a node $i \notin Y^{(n)}$ is unchanged after applying $F_n$, for a node $1 \leq j \leq n$, if $d_{\bG}(j, i) > k$ for all $i \in \cup_{t \in \vermark} Y^{(n)}_t$, the mark of all vertices in $(\bG,j)_k$ are unchanged after applying $F_n$ and $[\bG, j]_k \equiv [\bG', j]_k$. However, there are at least $n - \sum_{t \in \vermark} |Y^{(n)}_t| r_t$ many vertices satisfying this condition. Hence, using Lemma~\ref{lem:local-isomorphism-LP-distance} in Section~\ref{sec:coding-step-1-restriction-max-degree}, 
\begin{equation*}
  \dlp(U(\bG), U(\bG')) \leq \max \left \{ \frac{1}{k} , \frac{1}{n} \sum_{t \in \vermark} |Y^{(n)}_t|r_t \right \}.
\end{equation*}
Since $|Y^{(n)}_t| = o(n)$ for all $t \in \vermark$, we can choose $n$ large enough such that the above upper bound is no more than $1/k < 2 \epsilon$. To sum up, we have shown that if $\bG$ is a good graph,  $\dlp(U(\bG), U(F_n(\bG))) < 2 \epsilon$. This shows that if $\bG \in \mG'^{(n)}_{\bm_n, \bu_n}(\mu, \epsilon)$ is good, then $F_n(\bG) \in \mG'^{(n)}_{\bm_n, \tilde{\bu}_n}(\mu, 3\epsilon)$. 

Now we show that a sufficiently large fraction of  graphs in $\mG'^{(n)}_{\bm_n, \bu_n}(\mu, \epsilon)$ are good. For now, we assume that the set $\mG'^{(n)}_{\bm_n, \bu_n}(\mu, \epsilon)$ is not empty. Later we will discuss how to handle the case where $\mG'^{(n)}_{\bm_n, \bu_n}(\mu, \epsilon)$ is empty.
Let $\bG$ be drawn uniformly at random from the set $\mG'^{(n)}_{\bm_n, \bu_n}(\mu, \epsilon)$. Moreover, for $1 \leq i \leq n$, define the random variable $X_i$ to be 1 if $[\bG, i]_k \notin A^t_{k, r_t}$,  where $t$ is the mark of vertex $i$ in $\bG$. Otherwise, define $X_i$ to be zero. Invariance of $U(\bG)$ under vertex relabeling implies that for a permutation $\pi \in S_{\bu_n}$ and  $\bG \in \mG'^{(n)}_{\bm_n, \bu_n}(\mu, \epsilon)$, $\pi \bG \in \mG'^{(n)}_{\bm_n, \bu_n}(\mu, \epsilon)$. This means that 
\begin{equation}
  \label{eq:X-i-S-un-invariant}
  (X_{\pi(i)})_{1 \leq i \leq n} \stackrel{d}{=} (X_i)_{1 \leq i \leq n} \qquad \forall \pi \in S_{\bu_n},
\end{equation}
where $\stackrel{d}{=}$ denotes equality in distribution. Note that $\bG$ is good if and only for all  $i \in Y^{(n)}$, $X_i = 0$. On the other hand, if $\bG \in \mG'^{(n)}_{\bm_n, \bu_n}(\mu, \epsilon)$,  for all $t \in \vermark$, 
\begin{equation*}
  \mu(A^t_{k, r_t}) \leq U(\bG) \left ( \left(A^t_{k, r_t}\right)^\epsilon \right) + \epsilon.
\end{equation*}
But since $\epsilon < 1/(1+k)$, $(A^t_{k, r_t})^\epsilon = A^t_{k, r_t}$. By the definition of $r_t$, this means that $|J^{(n)}_t(\bG)| \geq n(\pi_t - 2 \epsilon$). 
Since $\epsilon< \pi_t / 2$, $\pi_t - 2 \epsilon > 0$ for all $t$.
As a result,
\begin{equation}
\label{eq:sum-Xi-upper-bound-li}
  \sum_{i \in I^{(n)}_t} X_i \leq \bu_n(t) - n \pi_t + 2n\epsilon \qquad \forall t \in \vermark.
\end{equation}
Now fix integers $l_1, \dots l_{|\vermark|}$ such that $0 \leq l_i \leq \bu_n(t_i) - n \pi_{t_i} + 2n\epsilon$ for all $1 \leq i \leq |\vermark|$. Then,  \eqref{eq:X-i-S-un-invariant} implies that  conditioned on the event $\sum_{j \in I^{(n)}_{t_i}} X_j = l_i$ for $1 \leq i \leq |\vermark|$, the sequence $X_1, \dots, X_n$ is uniformly distributed among the zero--one sequences with precisely $l_i$ many ones in $I^{(n)}_{t_i}$, for $1 \leq i \leq |\vermark|$.  
As $|Y^{(n)}| = o(n)$, we can choose $n$ large enough such that $l_i \leq \bu_n(t) - |Y^{(n)}_{t_i}|$, for all $1 \leq i \leq |\vermark|$. With such $n$, we have 
\begin{align*}
  \pr{X_j = 0\,\, \forall  j \in Y^{(n)} \Bigg| \sum_{j \in I^{(n)}_{t_i}} X_j = l_i, \forall 1 \leq i \leq |\vermark|} &= \frac{\prod_{i = 1}^{|\vermark|}\binom{\bu_n(t_i) - |Y^{(n)}_{t_i}|}{l_i}}{\prod_{i = 1}^{|\vermark|}\binom{\bu_n(t_i)}{l_i}} \\
&= \prod_{i = 1}^{|\vermark|} \frac{\bu_n(t_i) - |Y^{(n)}_{t_i}|}{\bu_n(t_i)} \times \dots \times \frac{\bu_n(t_i) - |Y^{(n)}_{t_i}| - l_i + 1}{\bu_n(t_i) - l_i + 1} \\
&\geq \prod_{i = 1}^{|\vermark|} \left ( \frac{\bu_n(t_i) - |Y^{(n)}_{t_i}| - l_i + 1}{\bu_n(t_i) - l_i + 1} \right )^{l_i} \\
&\geq \prod_{i = 1}^{|\vermark|} \left ( \frac{n(\pi_{t_i} - 2\epsilon) - |Y^{(n)}_{t_i}| + 1}{n(\pi_{t_i} - 2\epsilon) + 1} \right)^{\bu_n(t_i) - n(\pi_{t_i} - 2\epsilon)}
\end{align*}
where the last inequality follows from the fact that each term is decreasing in $l_i$ and $l_i \leq \bu_n(t_i) - n\pi_{t_i} +2n\epsilon$. Since this lower bound is uniform over $l_i$, we have 
\begin{equation}
  \label{eq:pr-G-good}
  \pr{\bG \text{ is good}} = \pr{X_j = 0 \,\, \forall j \in Y^{(n)}} \geq \prod_{i = 1}^{|\vermark|} \left ( \frac{n(\pi_{t_i} - 2\epsilon) - |Y^{(n)}_{t_i}| + 1}{n(\pi_{t_i} - 2\epsilon) + 1} \right)^{\bu_n(t_i) - n(\pi_{t_i} - 2\epsilon)} =: \alpha_n.
\end{equation}
As $\bG$ was chosen uniformly at random in $\mG'^{(n)}_{\bm_n, \bu_n}(\mu, \epsilon)$, this means that a $\alpha_n$ fraction of graphs in $\mG'^{(n)}_{\bm_n, \bu_n}(\mu, \epsilon)$ are good. This together with the fact that if $\bG$ is good, $F(\bG) \in \mG'^{(n)}_{\bm_n, \tilde{\bu}_n}(\mu, 3\epsilon)$ implies that 
\begin{align*}
  \log |\tilde{\bG}^{(n)}_{\bm_n, \tilde{\bu}_n} (\mu, 3\epsilon) | &\geq \log |\tilde{\bG}^{(n)}_{\bm_n, \bu_n} (\mu, \epsilon) | + \log \alpha_n  \\
&= \log |\tilde{\bG}^{(n)}_{\bm_n, \bu_n} (\mu, \epsilon) | + n \left ( \sum_{i=1}^{|\vermark|} \left ( \frac{\bu_n(t_i) - \pi_{t_i}}{n} +2\epsilon \right ) \log \left ( 1 - \frac{|Y^{(n)}_{t_i}|}{n(\pi_{t_i} - 2\epsilon) + 1} \right ) \right )
\end{align*}
Earlier we had made the assumption that $\mG'^{(n)}_{\bm_n, \bu_n}(\mu, \epsilon)$ is not empty to obtain the above inequality. But if $\mG'^{(n)}_{\bm_n, \bu_n}(\mu, \epsilon)$ is empty, the RHS is $-\infty$ and the above inequality still remains to hold. 
On the other hand, $|Y^{(n)}_{t_i}| / n \rightarrow 0$ for all $1 \leq i \leq |\vermark|$ and $\bu_n(t_i) / n \rightarrow \pi_{t_i}$; hence, subtracting $\norm{\bm_n}_1 \log n$ from both sides, dividing by $n$,  taking limsup over $n$ and then sending $\epsilon$ to zero, the second term in RHS vanishes and we get  $\bchover'^{(2)}_{\bd, \pi}(\mu) \geq \bchover'^{(1)}_{\bd, \pi}(\mu)$. Changing the order of $\bu_n$ and $\tilde{\bu}_n$, we get $\bchover'^{(2)}_{\bd, \pi}(\mu) =\bchover'^{(1)}_{\bd, \pi}(\mu)$. Substituting $\limsup$ with $\liminf$ we get  $\bchunder'^{(2)}_{\bd, \pi}(\mu) =\bchunder'^{(1)}_{\bd, \pi}(\mu)$. This completes the proof. 
\end{proof}


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "UniversalGraphCompression_arXiv"
%%% End: 

